Resilient Federated Learning under Byzantine Attack in Distributed Nonconvex Optimization with 2-f Redundancy

We study the problem of Byzantine fault tolerance in a distributed optimization setting, where there is a group of $N$ agents communicating with a trusted centralized coordinator. Among these agents, there is a subset of $f$ agents that may not follow a prescribed algorithm and may share arbitrarily incorrect information with the coordinator. The goal is to find the optimizer of the aggregate cost functions of the honest agents. We will be interested in studying the local gradient descent method, also known as federated learning, to solve this problem. However, this method often returns an approximate value of the underlying optimal solution in the Byzantine setting. Recent work showed that by incorporating the so-called comparative elimination (CE) filter at the coordinator, one can provably mitigate the detrimental impact of Byzantine agents and precisely compute the true optimizer in the convex setting. The focus of the present work is to provide theoretical results to show the convergence of local gradient methods with the CE filter in a nonconvex setting. We will also provide a number of numerical simulations to support our theoretical results.

==> Conclusion_and_Future_work.tex <==
\section{Conclusion}\label{sec:Conclusion}
This paper addresses Byzantine fault-tolerance in federated local stochastic gradient descent using the existing comparative elimination (CE) and study its fault-tolerance properties in both deterministic and stochastic settings when the local functions satisfy PL condition. In the deterministic setting, we prove that the CE filter achieves exact fault-tolerance against a bounded fraction of Byzantine agents $f/N$, provided the non-faulty agents' costs satisfy the necessary 2f-redundancy condition. In the stochastic setting, we show that the CE filter achieves approximate fault-tolerance, where the approximation error is proportional to the variance of the agents' stochastic gradients and the fraction of Byzantine agents.
